Fighting Online Click-Fraud Using Bluff Ads

Online advertising is currently the greatest source of revenue for many Internet giants. The increased number of specialized websites and modern profiling techniques, have all contributed to an explosion of the income of ad brokers from online advertising. The single biggest threat to this growth, is however, click-fraud. Trained botnets and even individuals are hired by click-fraud specialists in order to maximize the revenue of certain users from the ads they publish on their websites, or to launch an attack between competing businesses. In this note we wish to raise the awareness of the networking research community on potential research areas within this emerging field. As an example strategy, we present Bluff ads; a class of ads that join forces in order to increase the effort level for click-fraud spammers. Bluff ads are either targeted ads, with irrelevant display text, or highly relevant display text, with irrelevant targeting information. They act as a litmus test for the legitimacy of the individual clicking on the ads. Together with standard threshold-based methods, fake ads help to decrease click-fraud levels.

==> abstract.tex <==
Online advertising is currently the greatest source of revenue for many Internet giants. The increased number of specialized websites and modern profiling techniques, have all contributed to an explosion of the income of ad brokers from online advertising. The single biggest threat to this growth, is however, click-fraud. Trained botnets and even individuals are hired by click-fraud specialists in order to maximize the revenue of certain users from the ads they publish on their websites, or to launch an attack between competing businesses.

In this note we wish to raise the awareness of the networking research community on potential research areas within this emerging field. As an example strategy, we present \textit{Bluff ads}; a class of ads that join forces in order to increase the effort level for click-fraud spammers. Bluff ads are either targeted ads, with irrelevant display text, or highly relevant display text, with irrelevant targeting information. They act as a litmus test for the legitimacy of the individual clicking on the ads. Together with standard threshold-based methods, fake ads help to decrease click-fraud levels.

==> conclusion.tex <==
\section{Future Directions and Conclusions}
\label{sec:conclusion}

In this paper we presented a brief overview of the current challenges in detection of click-fraud in online advertising. We presented a simple detection strategy, Bluff ads. These are sets of irrelevant ads displayed amongst user's targeted ads, which should never be clicked on. Together with threshold detection, IP address monitoring and profile matching techniques, bluff ads can be used to make it more complicated for the botnet owners to train their software, or a human operator. The bluff ads also may have a comfort factor of decreasing the user's negative perceptions by reducing the number of accurately targeted ads. We are working on deployment of bluff ads on a large network ad service. We are also hoping to design more sophisticated bluff ads in order to avoid a trained bot to easily detect their irrelevancy based on dictionary look-ups.

The current solutions to click-fraud do not detect attacks by a malicious broker. In the current advertising models, one has to fully trust the broker. There are proposals for move away from a  broker-centric model~\cite{guha.hotnets09}. However until a practical solution is deployed, research is required to minimize the impact of click-fraud on businesses.

The click-fraud issue is a new and evolving area of work, both by click-fraud investigation teams, and by attackers. We need more datasets of ad clicks, better methods of battling attacks and large scale experiments on current methods such as Bluff ads. There are click-fraud schemes in which the publisher use only real clicks, but in a way that causes the broker to pay when it should not need to do so~\cite{ffsearch}. These attacks are done by hijacking search results form \url{google.com} for example, and displaying results which are brought to the user by \url{google.com}, while in reality redirecting the search and click traffic through an attacker's website and hence claiming referral bonus from Google. In this way the user does not notice any difference in results and the conventional methods of fraud detection are hardly useful. More research from the networking community is required to understand and battle such attacks without relying on the user's spyware detection software. 






==> fraudtype.tex <==
\section{Click fraud scenarios}
\label{sec:types}


Traditionally, online advertisers used the Cost-Per-Impression (CPI) model to charge for advertisements. The CPI is often measured in terms of the cost of one thousand impressions of the ad. These ads can be videos, images and links. Recently, search engines such as Google have given rise to the Pay-Per-Click (PPC) model for online advertising. In this type of arrangement, advertisers pay a certain amount of money to the publisher for every click on their ad (which leads to the advertiser's website). This model has however led to the rise of click fraud where users, or a botnet of computers fraudulently click on the ads in order to generate revenue for the publisher in an undetectable manner. Anupam~\etal~\cite{fraud} present a study on difficulty of detecting such attacks which demonstrates the difficulty of detecting click frauds. A deceitful publisher puts a script on his website that is automatically downloaded onto a visitor's computer when said visitor goes to the publisher's website. The script then imitates a click onto the advertisement leaving the visitor none the wiser. The log files of the advertiser (and, if applicable, of the publisher) will show the visitor's IP address. 

Other forms of click fraud include Competitors of advertisers, vandalism fans and friends of the publisher.\footnote{See \url{http://en.wikipedia.org/wiki/Click_fraud} for a detailed description}

It is quite hard for a botnet to launch a widely distributed clicking campaign realistically. The brokers have profiles of where an advertisers' benign clickers come from, when, and how often they click. The botnet has to match this profile to avoid detection based on thresholds. The Bluff ads presented in this paper are means for detecting the nodes of a trained botnet.

Some frauds are just out of anger. In response to Google's recently announced plans to expand the tracking of users, the international anti-advertising magazine Adbusters proposes that users collectively embark on a civil disobedience campaign of intentional, automated click fraud in order to undermine Google's advertising program in order to force Google to adopt a pro-privacy corporate policy. They have released a GreaseMonkey script that automatically clicks on all AdSense ads.\footnote{\url{http://yro.slashdot.org/article.pl?sid=09/03/12/2139258&from=rss}}




% A secondary source of click fraud is non-contracting parties, who are not part of any pay-per-click agreement. This type of fraud is even harder to police, because perpetrators generally cannot be sued for breach of contract or charged criminally with fraud. Examples of non-contracting parties are:
% 
%     * Competitors of advertisers: These parties may wish to harm a competitor who advertises in the same market by clicking on their ads. The perpetrators do not profit directly but force the advertiser to pay for irrelevant clicks, thus weakening or eliminating a source of competition.
%     * Competitors of publishers: These persons may wish to frame a publisher. It is made to look like the publisher is clicking on its own ads. The advertising network may then terminate the relationship. Many publishers rely exclusively on revenue from advertising and can be put out of business by such an attack.
%     * Other malicious intent: As with vandalism, there is an array of motives for wishing to cause harm to either an advertiser or a publisher, even by people who have nothing to gain financially. Motives include political and personal vendettas. These cases are often the hardest to deal with, since it is difficult to track down the culprit, and if found, there is little legal action that can be taken against them.
%     * Friends of the publisher: Sometimes upon learning a publisher profits from ads being clicked, a supporter of the publisher (like a fan, family member, or personal friend) will click on the ads to help. This can be considered patronage. However, this can backfire when the publisher (not the friend) is accused of click fraud.
% 
% Advertising networks may try to stop fraud by all parties but often do not know which clicks are legitimate. Unlike fraud committed by the publisher, it is difficult to know who should pay when past click fraud is found. Publishers resent having to pay refunds for something that is not their fault. However, advertisers are adamant that they should not have to pay for phony clicks.
% 
% 
% One type of fraud that circumvents detection based on IP patterns is one that uses existing user traffic, turning this into clicks or impressions [1] Such an attack can be camouflaged from users by using 0-size iframes to display advertisements that are programmatically retrieved using JavaScript. It could also be camouflaged from advertisers and portals by ensuring that so-called "reverse spiders" are presented with a legitimate page, while human visitors are presented with a page that commits click fraud. The use of 0-size iframes and other techniques involving human visitors may also be combined with the use of incentivized traffic, where members of "Paid to Read" sites are paid small amounts of money (often a fraction of a cent) to visit a website and/orclick on keywords and search results, sometimes hundreds or thousands of times every day [2] Some owners of PTR sites are members of PPC engines and may send many email ads to users who do search, while sending little ads to those who do not. They do this mainly because the charge per click on search results is often the only source of revenue to the site. This is known as forced searching, a practice that is frowned upon in the Get Paid To industry.
% 
% Organized crime can handle this by having many computers with their own Internet connections in different geographic locations. Often, scripts fail to mimic true human behavior, so organized crime networks use Trojan code to turn the average person's machines into zombie computers and use sporadic redirects or DNS cache poisoning to turn the oblivious user's actions into actions generating revenue for the scammer. It can be difficult for advertisers, advertising networks, and authorities to pursue cases against networks of people spread around multiple countries.
% 
% 
% Healthinsurancebids.com offers a revealing entry point into the click-fraud realm. It is one of several parked sites registered to Roland Kiss of Budapest. Kiss also owns BestPTRsite.com. "PTR" refers to "paid to read." In theory, paid-to-read sites recruit members who agree to read marketing e-mails and Web sites tailored to their interests. PTR site operators pay members for each e-mail and Web site they read, usually a penny or less.
% 
% In reality, many PTR sites are click-fraud rings, some with hundreds or thousands of participants paid to click on ads. BestPTRsite says it has 977 members. On Aug. 23 its administrator sent an e-mail to members containing a list of parked sites filled with ads. One of these sites, mortgagebg.com, which is also registered to Kiss, has been a source of apparently bogus clicks on MostChoice. The e-mail instructed members to click on different links every day, a common means to avoid detection. Members were also told to cut and paste text from the Web pages they click as proof of their activity. "If you send us back always the same link you will get banned and not paid! So take care and visit everyday a new link," the e-mail said. \texttt{www.wordlinx.com}



==> intro.tex <==
\section{Introduction}
\label{sec:intro}

Spending on Internet ads is growing faster than any other sector of the advertising industry and is expected to surge from \$12.5 billion last year to \$29 billion in 2010 in the U.S. alone, according to researcher eMarketer Inc. This trend is similar on the revenue form Internet activities when compared to the downfall of transit charges for example~\cite{atlas2009}. Most academics and consultants who study online advertising estimate that 10\% to 15\% of ads in pay per click online advertising systems are not authentic.\footnote{\url{http://www.businessweek.com/magazine/content/06_40/b4003001.htm}} The clicks are believed to be instantiated by users in poor countries, or botnets, who are trained to click on specific ads. This process is called click-fraud.

Click fraud is the subject of some controversy and increasing litigation due to the advertising networks being a key beneficiary of the fraud. On one hand, the brokers do not wish to lose customers. On the other hand, they are not able to provide full details of the clicks, their rates, and origin IP addresses to advertisers. Even worse, the advertisers would wish to claim that all clicks are fraud, hence avoiding click charges. For instance, broker loses money to undetected click fraud when it pays out to the publisher (third party website), but it makes more money when it collects fees from the advertiser. Because of the spread between what the broker collects and what it pays out, click fraud may directly profit the broker. This also provides an incentive for the publishers to hire click fraud botnets or human teams to increase their revenue.

Brokers claim they filter out most questionable clicks and either not charge for them or reimburse advertisers that have been wrongly billed. However this is a hard task, despite the claims that brokers' efforts are satisfactory~\cite{Tuzhilin}. On its simplest form, a weblog publisher continuously clicks on the ads displayed on his own website in order to make revenue. In a more complicated scenario, a hardware store may hire a large, globally distributed botnet in order to click on its competitors ads, hence depleting their daily budget. 

Another form of such fraud is view-fraud. In this case, a blogger may hire a botnet to continuously access its pages and retrieve ads without clicking on them, in long term generating revenue from ad impressions (views). Although the views are much cheaper than clicks, a high view to click ratio will usually affect the ad quality score and will drop the ad from the top spots, as the broker is interested in ads which generate clicks and bring in more revenue. 

Detecting click fraud is a relatively new area of research. On the simplest form, the broker performs threshold-based detection. If a web page is receiving a high number of clicks from the same IP address in a short interval, these clicks can be flagged as fraud. This gets more complicated if the clickers are behind proxies or globally distributed. In such cases the broker has to use global IP blacklists and continually update its list as the botnets evolve. 

In this paper we present \textit{Bluff Ads}, a set of ads which are designed to be detected and clicked only by machines, or poorly trained click-fraud work force. These ads are targeted at the same audience profile as the other ad groups, however their displayed text is totally unrelated to the user profile. Hence they should not be clicked on by the benign user. This simple set of ads, mixed with ordinary ads, work as a litmus test, or a ``Captcha'' for the user legitimacy. If a high number of them is clicked, the user is deemed to be flagged as suspicious. Another form of Bluff ads is a set which contain specialized text but they are not targeted to a specific profile and are randomly displayed. This group help detect click-fraud when the botnet builds up fake profile in order to harvest relevant ads.

We wish to insist that Bluff ads are, by no means, the ultimate defense against click-fraud. In fact this paper is a report on the status quo on click-fraud and detection mechanisms which raise the bar for attackers. We wish to inspire the network security and research community as a whole to pursue further research on advertising, release more datasets (such as Yahoo$!$ Webscope data\footnote{\url{http://webscope.sandbox.yahoo.com/}}) and devise strategies for privacy preserving advertising which also minimize click fraud.





==> related.tex <==
\section{Related Work}
\label{sec:related}


There are a  number of solutions for avoiding click fraud and performing better advertisement. One suggestion is to charge based on user's actions, i.e., the publisher gets a premium only after the successful conversion of the ad, meaning the user's visit to the advertiser website and performing an action such as buying an item or signing up for a service. There are a number of basic attempts at such approach by means of tracking cookies, however these efforts make up a negligible portion of the current advertising revenue on the Internet.

Juels~\etal~\cite{juel_prem} propose a cryptographic approach for replacing the pay-per-click model with one in which pay-per-action (e.g., shopping) can attract premium rates and unsuccessful clicks are discarded. in this system, the users which make a purchase are identified by the network of advertisers as premium advertisers. The client browsers use a coupon instantiated by third party cookies or issued by the attestor upon redirection. The disadvantage of this method is the ability of malicious attacker, possibly an advertiser, to use a botnet and replay the coupons numerous times, for a large number of cooperating publishers. This will then force the syndicator either discount all those replays, or removing those clients form the system with valid coupons. In both cases, the advertisement income is minimized. It also allows for the syndicator and the attestor (ad broker and middle box) to profile the users accurately including their spending budget. They also indicate that most standard click fraud techniques remain unsolved today. Despite early suggestions of this method, it has not been implemented on a large scale as it requires trust between advertisers and publishers. 

Some advertisers have suggested the use of anonymised ISP data stream for verification of clicks and for better user profiling. However such attempts have been unsuccessful due to user privacy concerns. Privacy reasons also prevent brokers from releasing their server logs and click data to advertisers and their agents for deep inspection of the click rates. Other solutions include use of human-invisible ads to act as traps for botnets, however these can easily be ignored by a simple visibility test in botnet design.

Immorlica~\etal~\cite{immorlica2005clickfraud} analyze the click fraud learning algorithms to compute the estimated click-through rate. They focus on a situation in which there is just one ad slot, and show that fraudulent clicks can not increase the expected payment per impression by more than o(1) in a click-based algorithm. However the complexity of the inferred algorithm and the need for click-through rate estimation would make it impractical as it also deviates form the pay per click model, to pay per view model, which is the least desired model in the modern advertisement world where bidding for space is of critical importance.



